Inferring Tracker-Advertiser Relationships in the Online Advertising Ecosystem using Header Bidding

Online advertising relies on trackers and data brokers to show targeted ads to users. To improve targeting, different entities in the intricately interwoven online advertising and tracking ecosystems are incentivized to share information with each other through client-side or server-side mechanisms. Inferring data sharing between entities, especially when it happens at the server-side, is an important and challenging research problem. In this paper, we introduce KASHF: a novel method to infer data sharing relationships between advertisers and trackers by studying how an advertiser's bidding behavior changes as we manipulate the presence of trackers. We operationalize this insight by training an interpretable machine learning model that uses the presence of trackers as features to predict the bidding behavior of an advertiser. By analyzing the machine learning model, we are able to infer relationships between advertisers and trackers irrespective of whether data sharing occurs at the client-side or the server-side. We are also able to identify several server-side data sharing relationships that are validated externally but are not detected by client-side cookie syncing.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

#full 	: all
#	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -sOutputFile=main_full.pdf -f main.pdf
#
full	: all
all 	: $(PDF)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

#$(PSF)	: %.ps : %.dvi
#	  @$(DVIPS) $< -o $@
#
#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
$(PDF) : %.pdf : %.tex
	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> measurement_tables.tex <==
\begin{table}[!t]
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline \multirow{2}{*}{} & {Num. Sites} &\multicolumn{2}{c|}{No Intent} & \multicolumn{2}{c|}{Intent} & \multicolumn{2}{c|}{Total Bids} \\
& & positive bids & zero bids & positive bids & zero bids &
\\
\cline{1-8}                                
appnexus& 13& 4756& 8& 3720& 2 & 8486 \\ \hline 
rubicon& 15& 3268& 120& 2928& 68 & 6384 \\ \hline
ix& 7& 2591& 0& 2235& 0 & 4826\\ \hline
openx& 9& 2376& 25& 2151& 5 & 4557\\ \hline
pubmatic& 13& 2444& 5376& 2060& 4065 & 13945 \\ \hline
criteo& 7& 1518& 94& 1538& 25 & 3175\\ \hline
indexExchange& 4& 1232& 905& 1159& 224& 3520\\  \hline
sovrn& 3& 876& 102& 970& 39& 1987\\ \hline
appnexusAst& 4& 1193& 11& 920& 10 & 2134 \\ \hline
aol& 6& 1164& 111& 872& 88 & 2235\\ \hline
conversant& 2& 107& 0& 773& 0 & 880\\ \hline
districtm& 2& 573& 0& 341& 0 & 914\\ \hline
triplelift& 2& 193& 0& 189& 0 & 382\\ \hline
lockerdome& 1& 202& 0& 187& 0 & 389\\ \hline
sonobi& 2& 43& 0& 66& 0 & 109\\ \hline
33across& 1& 89& 0& 52& 0 & 141\\ \hline
trustx& 3& 25& 18& 36& 8 & 87\\ \hline
smartadserver& 1& 47& 0& 17& 0 & 64\\ \hline
newsconnect& 1& 3& 0& 6& 0 & 9\\ \hline
innity& 2& 0& 480& 0& 344 & 824\\ \hline
Total & - &22700& 7250& 20220& 4878 & 55048\\ \hline
\end{tabular}
\caption {Number of bids collected for 20 bidders.}
\label{table:BIDVOLUME}
\end{table}
\begin{table}[!t]
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline Categories &  appnexus&	 rubicon&  ix&	 openx& pubmatic &	 Avg. \\
\hline 
Adult& 0.21& \textcolor{red}{\textbf{0.43}}& 0.25& 0.33& 0.34& 0.36 \\ \hline
Arts& 0.34& \textcolor{red}{\textbf{0.45}}& 0.29& 0.37& 0.36& 0.43 \\ \hline
Business& 0.28& 0.45& 0.28& 0.30& \textcolor{red}{\textbf{0.51}}& 0.42 \\ \hline
Computers& 0.20& \textcolor{red}{\textbf{0.75}}& 0.21& 0.55& 0.73*& 0.54 \\ \hline
Games& 0.21& 0.33& 0.21& \textcolor{red}{\textbf{0.34}}& 0.25& 0.31 \\ \hline
Health& 0.21& \textcolor{red}{\textbf{1.16}}*& 0.28& 0.94*& 0.54& \textcolor{red}{\textbf{0.70}} \\ \hline
Home& 0.20& \textcolor{red}{\textbf{0.39}}& 0.24& 0.28& 0.28& 0.33 \\ \hline
Kids\&Teens& 0.20& 0.41& 0.18& \textcolor{red}{\textbf{0.47}}& 0.30& 0.35 \\ \hline
News& 0.19& \textcolor{red}{\textbf{0.61}}& 0.24& 0.41& 0.33& 0.41 \\ \hline
Recreation& 0.31& \textcolor{red}{\textbf{0.67}}& 0.23& 0.36& 0.44& 0.48 \\ \hline
Reference& 0.18& 0.53& 0.20& 0.52& \textcolor{red}{\textbf{0.58}}& 0.44 \\ \hline
Regional& 0.23& 0.43& 0.33& \textcolor{red}{\textbf{0.73}}& 0.35& 0.45 \\ \hline
Science& 0.30& \textcolor{red}{\textbf{0.70}}& 0.28& 0.44& 0.58& 0.53 \\ \hline
Shopping& 0.40*& 0.56& 0.45*& 0.47& \textcolor{red}{\textbf{0.60}}& 0.58 \\ \hline
Society& 0.22& 0.41& 0.27& \textcolor{red}{\textbf{0.45}}& 0.37& 0.39 \\ \hline
Sports& 0.19& \textcolor{red}{\textbf{0.35}}& 0.13& 0.23& 0.30& 0.28 \\ \hline
Control& 0.20& 0.26& 0.28& \textcolor{red}{\textbf{0.44}}& 0.37& 0.35 \\ \hline
Avg.& 0.24& \textcolor{red}{\textbf{0.52}}& 0.26& 0.45& 0.42& 0.43 \\ \hline
\end{tabular} \label{table:BIDVALUES}
\caption {Header Bidding median CPMs (USD) across 17 profiles. Max bids for each category bolded red, `*' following bid indicates the category of bidder paid the highest price.}
\end{table}
\begin{table*}[!t]
\scriptsize
\begin{tabular}{|c|c|c|c|}  \cline{1-4}
\hline
Appnexus & Shopping& Arts& Recreation \\ \hline
Rubicon& Health& Computers& Science \\ \hline
IX& Shopping& Regional& Arts \\ \hline
OpenX& Health& Regional& Computers  \\ \hline
Pubmatic& Games& Society& Regional  \\ \hline
\end{tabular}
\caption{Top three most-valued categories no-intent web personas}
\label{table:BIDCPMSCAT}
\end{table*}
\begin{table*}[!t]
\caption{Ratio of intent bids prices to no intent bid prices. Max ratios for each category bolded red, `*' following ration's indicates the category max ration of a bidder}

\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}  \cline{1-7}
\hline
Bidders& appnexus& rubicon& ix& openx& pubmatic& Avg.\\ \hline
Adult& 0.97& 0.97& \textcolor{red}{\textbf{2.10}}& 0.85& 0.95& 1.12 \\ \hline
Arts& 1.04& \textcolor{red}{\textbf{1.49}}& 1.45& 0.97& 1.32& 1.26 \\ \hline
Business& 1.02& 1.09& \textcolor{red}{\textbf{2.66}}& 1.01& 0.84& 1.24 \\ \hline
Computers& 1.06& 1.19& \textcolor{red}{\textbf{2.38}}& 1.18& 0.71& 1.14 \\ \hline
Games& 1.20& \textcolor{red}{\textbf{1.83}}& 1.81& 1.06& 1.80*& 1.53 \\ \hline
Health& 1.85*& 1.25& 1.34& \textcolor{red}{\textbf{5.96}}*& 1.21& \textcolor{red}{\textbf{2.70}} \\ \hline
Home& 1.31& 0.92& \textcolor{red}{\textbf{1.50}}& 1.12& 1.21& 1.17 \\ \hline
Kids\&Teens& 1.31& 1.52& \textcolor{red}{\textbf{6.00}}*& 0.76& 1.49& 1.78 \\ \hline
News& 1.05& 1.14& \textcolor{red}{\textbf{3.57}}& 1.05& 0.95& 1.40 \\ \hline
Recreation& \textcolor{red}{\textbf{1.76}}& 1.09& 1.04& 1.08& 0.86& 1.13 \\ \hline
Reference& 1.02& 1.06& \textcolor{red}{\textbf{2.80}}& 0.70& 0.60& 1.00 \\ \hline
Regional& 1.04& \textcolor{red}{\textbf{2.24}}& 1.46& 0.96& 0.83& 1.29 \\ \hline
Science& 1.11& 1.03& 0.81& 1.12& 0.92& 1.00 \\ \hline
Shopping& 1.18& 1.42& \textcolor{red}{\textbf{1.55}}& 1.52& 1.00& 1.32 \\ \hline
Society& 1.30& 2.16& \textcolor{red}{\textbf{2.52}}& 0.76& 0.92& 1.47 \\ \hline
Sports& 1.13& 3.00*& \textcolor{red}{\textbf{3.69}}& 2.85& 1.57& 1.47 \\ \hline
Control& 0.87& 1.32& \textcolor{red}{\textbf{1.33}}& 0.60& 0.92& 0.97 \\ \hline
Avg& 1.19& 1.45& \textcolor{red}{\textbf{2.24}}& 1.39& 1.07& 1.35 \\ \hline
\end{tabular}
\label{table:BIDRATIOS}
\end{table*}
\begin{table*}[!t]
\scriptsize
\begin{tabular}{|c|c|c|c|}  \cline{1-4}
\hline
Appnexus & Health & Recreation & Kids\&Teens \\ \hline
Rubicon & Sports & Regional & Society \\ \hline
IX & Kids\&Teens & Sports &  News\\ \hline
OpenX & Health & Sports & Shopping \\ \hline
Pubmatic & Games & Sports & Kids\&Teens \\ \hline
All Bidders & Health & Kids\&Teens  & Games \\ \hline
\end{tabular}
\caption{Top three most-valued categories intent web personas}
\label{table:BIDRATIOSCAT}
\end{table*}





